Exploring and Exploiting Diversity for Image Segmentation

Semantic image segmentation is an important computer vision task that is difficult because it consists of both recognition and segmentation. The task is often cast as a structured output problem on an exponentially large output-space, which is typically modeled by a discrete probabilistic model. The best segmentation is found by inferring the Maximum a-Posteriori (MAP) solution over the output distribution defined by the model. Due to limitations in optimization, the model cannot be arbitrarily complex. This leads to a trade-off: devise a more accurate model that incorporates rich high-order interactions between image elements at the cost of inaccurate and possibly intractable optimization OR leverage a tractable model which produces less accurate MAP solutions but may contain high quality solutions as other modes of its output distribution. This thesis investigates the latter and presents a two stage approach to semantic segmentation. In the first stage a tractable segmentation model outputs a set of high probability segmentations from the underlying distribution that are not just minor perturbations of each other. Critically the output of this stage is a diverse set of plausible solutions and not just a single one. In the second stage, a discriminatively trained re-ranking model selects the best segmentation from this set. The re-ranking stage can use much more complex features than what could be tractably used in the segmentation model, allowing a better exploration of the solution space than simply returning the MAP solution. The formulation is agnostic to the underlying segmentation model (e.g. CRF, CNN, etc.) and optimization algorithm, which makes it applicable to a wide range of models and inference methods. Evaluation of the approach on a number of semantic image segmentation benchmark datasets highlight its superiority over inferring the MAP solution.

==> CHANGES <==
Changes in version 4.3 (tbd)
o When redefining the acronym label, check for the 
  acronym package's version (thanks to Scott Lowe)
o Several minor fixes (comments, whitespaces removed,
  .gitignore, .editorconfig, etc.; thanks to Jörn 
  Hees) 
o Updated comments regarding hyperref's draft option 
  (thanks to Claudio Diaspero)
o Silenced the warnings from KOMA and titlesec about 
  each other, also in the examples (thanks to Jörg 
  Weber)

Changes in version 4.2 (September 2015)
o Fixed issue between titlesec and tocloft regarding
  part numbering in the ToC (classicthesis.sty).
  Thanks to Enrico Gregorio and Henri Menke.
o Fixed bug with colored lines and graffiti
  (classicthesis.sty). Thanks to Enrico Gregorio and
  Stefano Bragaglia for the fix! (Also switched
  graffiti from \slshape to \itshape.)
o Changed \vspace*{8ex} to \vspace{8ex} (Contents.tex)
o Moved \cleardoublepage from end of Contents.tex
  to appropriate position in ClassicThesis.tex
o \bflabel of acronym package removed, as it was
  removed from acronym package and caused errors.
  Now set \aclabelfont to \acsfont for consistency.
o Converted major files to UTF-8 (thanks to Jörn Hees)
  (Bibliography.bib excluded for now as BibTeX cannot
  handle UTF-8)
o Added support for BibLaTeX in
  classicthesis-config.tex and Bibliography.tex
  (thanks to Jörn Hees).
  For LyX we will have a work-around for testing.
o Added an example for one's own publication list
  (via BibLaTeX) in Publications.tex (renamed from
  Publication.tex)
o Replaced/updated scrpage2 with scrlayer-scrpage
  in classicthesis.sty (thanks to Ivo Pletìkosić).
X Worked on Appendix case with floatperchapter
  (works for captions but not for references so far)
  Thanks to Claus Lahiri and Clemens Niederberger
  for their help on this.
  [REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]
X Removed fixltx2e from classicthesis-config.tex and
  have classicthesis.sty use or emulate the latest
  LaTeX kernel via latexrelease (option: latest)
  (thanks to Jörn Hees).
  [REMOVED AS IT IS NOT AVAILABLE IN MANY
  DISTRIBUTIONS, SEE ISSUE #107]

Changes in version 4.1 (August 2012)
o Working towards XeLaTeX support:
  - "ifxetex" package for checking whether
    XeTeX is in use (classicthesis.sty)
  - Adjusted part, chapter, and tocEntry
  - Thanks to Joerg Weber for his ideas and code
  - Option "pdfspacing" does not work for XeTeX
    and is disabled when XeTeX is running
    (maybe implement spacing with fontspec later)
o Load additional packages in order to
  reduce warnings (classicthesis-config.tex)
  - "textcomp" to fix warnings with missing font
    shapes
  - "scrhack" to fix warnings when using KOMA
    with listings package
o Replaced \mathrm-command with \textrm-command
  (Chapter03.tex)

Changes in version 4.0 (December 2011)
o Due to lots of issues and complaints,
  classicthesis-preamble.sty is replaced by
  classicthesis-config.tex (which is cleaner,
  nicer, better, etc. than before!)
o No per-chapter-numbering also for equations
  (classicthesis.sty and Chapter03.tex)
o classicthesis.sty now also works without the
  KOMA-classes (scrbook, scrartcl, etc.):
  - This affects the text body shape, where the
    package "typearea" is always loaded in order
    to use \areaset
  - And affects the layout of footnotes where the
    package "footmisc" is loaded otherwise
    (not 100\% identical look-and-feel but OK)
o Help for using spanish babel with classicthesis
  (classicthesis-config.tex)
o Note about pdfsync issues with graffiti
  (Chapter01.tex)
o Minor clean-up of comments and duplicate lines
  (classicthesis.sty)
o Adjusted the colophon text (Colophon.tex)
o Increased space for labels in the LoF, LoT, LoL
o Included version information on the title page and
  in the drafting and final version information
  (classicthesis.sty and Titlepage.tex)

Changes in version 3.0 (June 2011)
o There have been some major changes in order to port
  classicthesis to LyX easily. See below for details.
  Special thanks go to Ivo Pletikosi\'c for all his
  hard work he put into this project!
o Changes in ClassicThesis.tex:
  - Redundant fleqn removed from documentclass options
   (will be set by amsmath package in preamble)
  - KOMA adjustments for documentclass:
    fontsize=11pt,paper=14
  - Moved language options into documentclass due to LyX
    issues with babel
o Changes in classicthesis.sty:
  - Removed bcor from \areaset command so that it can
    be set via \documentclass option (BCOR=)
  - New \ctparttext command for putting preamble text
    after part titles (see ClassicThesis.tex for examples)
  - \graffito command now also available as original
    \marginpar (backward compatibility is enabled)
  - Chapter number in margin done with \oldmarginpar
o Changes to classicthesis-preamble.sty:
  - Fixed autoref for subfigures (see Chapter 2 for example)
  - Fixed issues with redefining autoref strings (for
      different languages)
  - Now contains all configuration information, such as
    the title, your name etc.
  - This package now also loads classicthesis.sty, change
    the options classicthesis to be loaded with here
  - Package inputenc now loaded with latin9 option
  - Package listings now also loaded here
  - Now safer package loading regarding options by
    using \PassOptionsToPackage command extensively
  - Inserted new string for \mySubtitle
o Changes in Titlepage.tex and Titleback.tex because of new
  string \mySubtitle
o Changed a lot of the documentation, e.g., in Chapter01.tex

Changes in version 2.9 (January 2011)
o Fixed onlytext euler font for MinionPro font (in
  classicthesis.sty)
o Option "listsseparated" deprecated, because it led to some
  strange side-effects (in classicthesis.sty)
o Changed default font size to 11pt (in ClassicThesis.tex) and
  adjusted text block size accordingly (in classicthesis.sty)
o Fixed bug with backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o New option "floatperchapter" for classicthesis.sty, removed
  all code for that from classicthesis-ldpkg.sty
o Removed "nochapters" option from classicthesis-ldpkg.sty
o Removed redundant loading of listings package (in
  classicthesis-ldpkg.sty)
o Fixed some headline bug in example classicthesis-book.tex
o Fixed a bug when using parts with plain latex as in example
  classicthesis-book.tex (in classicthesis.sty)

Changes in version 2.8 (March/May 2010)
o Fixed serious \graffito bug in classicthesis.sty
  (thanks to Lorenzo Pantieri and Enrico Gregorio)
o Included backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o Fixed drafting issues (draft information not shown at all)
  caused by wrong code for listings and listsseparated options
  in classicthesis.sty

Changes in version 2.7 (February 2010, cumulative release)
o Removed option for classicthesis-ldpkg.sty: nobackref
  Introduced instead option "backref" for consistency
  which works the other way (no backrefs by default)

Changes in version 2.6.2 (January 2010, released as beta)
o New option for classicthesis-ldpkg.sty: nobackref
  (removes links to cited page in bibliography)
o Fixed some spacing issues for LoF, LoT, LoL with option
  "listsseparated" (in classicthesis.sty)

Changes in version 2.6.1 (October 2009, released as beta)
o Removed \myChapter and \myPart, you can now use the regular
  \chapter and \part commands (in classicthesis.sty)
  (thanks to Hinrich Harms for this)
o Fixed used KOMA-options: numbers=noenddot, cleardoublepage=empty
  (in ClassicThesis.tex)
o Included hack to use citations in float environments, will
  be fixed with caption package version 3.2 (in classicthesis.sty)
o Included some font and text area fine-tuning code
  (in ClassicThesis.tex)
o Some testing with Libertine font (classicthesis-book.tex)
o Fixed numbering of listings used in different chapters
  (in ClassicThesis.tex, classicthesis.sty, classicthesis-ldpkg.sty)
o Spacing between listings in different chapters and after List
  of Listings header fixed (in classicthesis.sty)
o Increased \newnumberwidth to sizeof(999) which is better for
  documents with more than 99 pages (in classicthesis.sty)
o New option for classicthesis.sty: manychapters

Changes in version 2.6 (August 2009)
o Centered the title page with the addmargin environment
  (thanks to Nicolas Repp for the hint)
o Fixed header for page two of Table of Contents (with 3
  or more pages) (in Contents.tex)
o Added numbering of \subsubsection (in Contents.tex)
o Added correct Table of Contents entries for \subsubsection
  (in classicthesis.sty)
o Added printonlyused option to loading acronym package
  (in classicthesis-ldpkg.sty)
o Some code for "clean" hyperlinks (w/o color and w/o boxes)
o Minor fix for \graffito (in classicthesis.sty)

Changes in version 2.5.1 (May 2009, released as beta)
o New option for classicthesis.sty: dottedtoc
  (Refer to the manual for more information.)
o New option for classicthesis.sty: listings
  (Refer to the manual for more information.)
  (Credit + thanks to Prof. Enrico Gregorio)
o Minor clean-up and bug-fixing

Changes in version 2.5 (October 2008, cumulative release)
o Increased text-width for better page layout (experimental)
o Cumulative release, some minor clean-up and bug-fixing

Changes in version 2.4.{1--3} (February and April 2008,
released as betas)
o Switched back to "obsolete" KOMA options due to
  compatibility issues on some installations
o Increased robustness of \cauthor command in
  classicthesis-ldpk.sty
o Spacing fix for \sectionmark (in classicthesis.sty)
o Made Booleans private (in classicthesis.sty)
o Acronyms header for long acronym lists (in Contents.tex)
o Moved "amsmath" package from classicthesis.sty to
  ClassicThesis.tex
o "MinionPro" package now loaded with "mathlf" option
  instead of "osf" option (in classicthesis.sty)
o Fixed issue with contents headings (in classicthesis.sty
  and in Contents.tex)
o Thanks to Lorenzo

Changes in version 2.3 (November 2007)
o Fixed serious bug with \myChapter command (using plain
  LaTeX)
o Removed hypcap package from classicthesis-ldpkg.sty and
  placeins package from classicthesis.sty. Put both into
  ClassicThesis.tex for finer end-user control
o Removed obsolete KOMA options from ClassicThesis.tex
o Option "subfigure" deprecated, replaced by "subfig" (in
  classicthesis.sty)
o Inserted some mechanisms to detect whether subfig(ure)
  package was loaded or not (in classicthesis.sty)
o Inserted some mechanism to detect whether classicthesis
  packackage was loaded or not (in classicthesis-ldpkg.sty)
o Moved "headlines" code block a bit up in
  classicthesis.sty (seemed to cause problems with new
  KOMA-Script classes)
o Removed accidental "natbib" from classicthesis-ldpkg.sty
o Some fine-tuning in (Dirty)Titlepage.tex
o Thanks to Lorenzo and Denis! :-)

Changes in version 2.2 (October 2007)
o \myChapter and \myPart now take an optional argument
  just as the regular \part and \chapter commands
o Did some minor changes to classicthesis-book.tex
  so it's a better example
o Inserted some \cleardoublepage before \myPart
  occurences to avoid pdfbookmark problems
o Introduced some general typographic fine-tuning
  (linespread, penalties, etc.)
o Did some fine-tuning of the \graffito command

Changes in version 2.1 (July 2007)
o Removed duplicate xcolor package call from
  classicthesis-ldpkg.sty and shifed some color
  definitions around
o Removed re-definition of \ttdefault

Changes in version 2.0 (June 2007, cumulative release)
o Better setup of the list of acronyms
  (in classicthesis-ldpkg.sty)
o Using KOMA option footinclude in ClassicThesis.tex
  (text block sizes are adjusted to this)
o New option for classicthesis.sty: minionpro
o New option for classicthesis.sty: minionprospacing
o New option for classicthesis.sty: pdfspacing
  (Refer to the manual for more information.)

Changes in version 1.7 (May 2007, not released separately)
o Removed \graphicspath from ClassicThesis.tex
o Use the nag package to ensure "compliance"
o Switched from ccaption to caption in classicthesis-ldpkg.sty
  (setup via \captionsetup in ClassicThesis.tex)
o Switched from subfigure to subfig in classicthesis-ldpkg.sty
o Removed obsolete "usenames" option from loading xcolor package
o Noticed problem with \thelstlisting on some installations
  (commented out in classicthesis-ldpkg.sty)
o Noticed problem with some hyperlinks on some installations
  (could not determine cause)

Changes in version 1.6 (April 2007, not released separately)
o Included greetings to Lorenzo Pantieri for many very useful
  suggestions
o Introduced new commands in classicthesis-ldpkg.sty to make
  adaptation of backrefs to different languages easier
   - \backrefnotcitedstring (ref is not cited)
   - \backrefcitedsinglestring (ref is cited on one page)
   - \backrefcitedmultistring (ref is cited on multiple pages)
o Removed ellipsis package from classicthesis-ldpkg.sty due to
  some undesired results for some users
o Removed the following packages from classicthesis-ldpkg.sty as
  these seem to require changes to their options from most users:
  inputenc, babel, natbib (now in ClassicThesis.tex)
o New option for classicthesis-ldpkg.sty: nochapters
  Use the package with classes that do not have chapter divisions

Changes in version 1.5 (April 2007, not released separately)
o Fixed some bugs to use classicthesis.sty for article layout
o Inserted some info/warnings when using nochapter/parts
o Extended the manual: examples for using classicthesis.sty for
  other projects than a thesis (source available in folder
  "Examples")
o Some minor adjustments in classicthesis-ldpkg.sty
o Fixed some spelling mistakes

Changes in version 1.4.2 (March 2007)
o Renamed loadpackages.sty to classicthesis-ldpkg.sty due to
  TeX Live package tree issues

Changes in version 1.4.1 (March 2007)
o Fixed some wording concerning the license :-o
o Added fixltx2e and ellipsis packages to to loadpackages.sty to correct
  some minor glitches
o Fixed and changed some things about ToC entries of parts
o Some minor bug fixes

Changes in version 1.4 (January 2007)
o Replaced \lineheight with \baselineskip in classicthesis.sty
o Removed obsolete "usenames" option from xcolor package (classicthesis.sty)
o Now classicthesis.sty processes the global a5paper option and adjusts
  the layout accordingly (experimental!)

Changes in version 1.3.1 (August 2006)
o Urgent bug concerning ToC spacing etc. fixed

Changes in version 1.3 (August 2006)
o New option for classicthesis.sty: parts
  Turn this on if you use Part divisions. It fine-tunes the ToC and
  adds support for Part division via \myPart{} (cf. \myChapter{})
  (The style of this feature is preliminary, any suggestions?!)
o New option for classicthesis.sty: eulermath
  Uses the awesome Euler fonts for math (Palatino fonts are default).
o Added mparhack package to loadpackages.sty to get the graffiti right
o Added a hint to loadpackages.sty on how to typeset the List of
  Listings consistently with classicthesis
o Some minor fine-tuning of typographic details
o Collaboration with babel package improved (now easier to use
  with other languages than English)
o Added appropriate textwidth values for 11pt Palatino and Minion
  (See comments near \areaset in classicthesis.sty)
o Note: There is a problem with the case of math text in part-,
  chapter-, and section titles and I have no clue how to fix this
  (either the case or the spacing breaks). So far, I chose the case. :-(

Changes in version 1.2 (June 2006)
o Setup a little postcard collection: http://postcards.miede.de
o Changed stupid spelling mistake: "A Homage" => "An Homage" D'oh!
o New option for classicthesis.sty: nochapters
  Allows to use the look-and-feel with classes that do not use chapters.
o New option for classicthesis.sty: beramono
  Loads Bera Mono as typewriter font. (Default = no typewriter font.)
o Included list of files, see LISTOFFILES.

Changes in version 1.1 (May 2006)
o classicthesis.sty now stand-alone and usable w/o whole bundle!
o classicthesis.sty compatible with both LaTeX and PDFLaTeX
  Note: this is only true for classicthesis.sty, not the whole bundle.
o New option for classicthesis.sty: subfigure
  Tells the style to add the respective option when loading tocloft.
o Now loading microtype package w/o options (classicthesis.sty)
o Fixed overfull hbox warnings for ToC entries (classicthesis.sty)
o No longer depending on a particular caption package (classicthesis.sty)
o Layout for subsubsections provided (classicthesis.sty)
o PDF opens on title page (ClassicThesis.[tex|pdf])
o Files are a bit more "ASCII-friendly" (all)
o Note: Thanks to all the folks who already sent me a postcard! :-)

Version 1.0 (March 2006)
o First public release


==> FrontBackmatter/Bibliography.tex <==
%********************************************************************
% Bibliography
%*******************************************************
% work-around to have small caps also here in the headline
\manualmark
\markboth{\spacedlowsmallcaps{\bibname}}{\spacedlowsmallcaps{\bibname}} % work-around to have small caps also
%\phantomsection
\refstepcounter{dummy}
\addtocontents{toc}{\protect\vspace{\beforebibskip}} % to have the bib a bit from the rest in the toc
\addcontentsline{toc}{chapter}{\tocEntry{\bibname}}
\label{app:bibliography}
\printbibliography

